TEAM: Trilateration for Exploration and Mapping with Robotic Networks

Motivated by lunar exploration, we consider deploying a network of mobile robots to explore an unknown environment while acting as a cooperative positioning system. Robots measure and communicate position-related data in order to perform localization in the absence of infrastructure-based solutions (e.g. stationary beacons or GPS). We present Trilateration for Exploration and Mapping (TEAM), a novel algorithm for low-complexity localization and mapping with robotic networks. TEAM is designed to leverage the capability of commercially-available ultra-wideband (UWB) radios on board the robots to provide range estimates with centimeter accuracy and perform anchorless localization in a shared, stationary frame. It is well-suited for feature-deprived environments, where feature-based localization approaches suffer. We provide experimental results in varied Gazebo simulation environments as well as on a testbed of Turtlebot3 Burgers with Pozyx UWB radios. We compare TEAM to the popular Rao-Blackwellized Particle Filter for Simultaneous Localization and Mapping (SLAM). We demonstrate that TEAM requires an order of magnitude less computational complexity and reduces the necessary sample rate of LiDAR measurements by an order of magnitude. These advantages do not require sacrificing performance, as TEAM reduces the maximum localization error by 50% and achieves up to a 28% increase in map accuracy in feature-deprived environments and comparable map accuracy in other settings.

==> old_related_work.tex <==
% 1. mapping unknown environments
% 1a. SLAM, Rao-Blackwellized particle filters
% 1b. map representations: occupancy grids
% 2. multi-robot mapping
% \cite{li2017corb}
% 2a. distributed perception
% 2b. virtual tether
% 3. cooperative positioning
% 3a. relative localization in sensor networks
% 3b. relative localization in robotics 
% 4. robotic mesh network testbeds
Robotic mapping of unknown environments is a well-researched field \cite{thrun2002robotic, kostavelis2015semantic, bresson2017simultaneous}. The closely related problem of localizing a robot within a map or coordinate frame is also well-researched, with methods including dead-reckoning, active beacons, GPS, landmark-based navigation, and map-matching \cite{borenstein1997mobile}. In mapping unknown environments, localization and mapping are often referred to as a ``chicken-and-egg" problem, wherein the robot must associate data to its position in order to map and associate its position to the map in order to localize. Many algorithms exist for handling this approach iteratively, referred to as Simultaneous Localization and Mapping (SLAM) \cite{durrant2006simultaneous1, bailey2006simultaneous2}. The authors of \cite{grisetti2007improved} present an improved Rao-Blackwellized Particle Filter (RBPF), a Monte Carlo localization algorithm which combines a proposal distribution for the robot's sensors and an adaptive resampling technique to improve the efficiency of previous SLAM methods. Available open source via the GMapping library \cite{gmapping}, this improved RBPF (referred to here as simply SLAM) is used as a benchmark localization and mapping algorithm for comparison in this work. 
% This algorithm, as well as the algorithm presented here, uses occupancy grid maps where each grid cell takes on one of three values: unknown, occupied, or free space. Other map representations including landmark-based maps and object/polygon maps exist and may be more suitable for certain applications.

% Localization \cite{borenstein1997mobile} dead-reckoning, reference-based systems (compasses, active beacons, GPS, landmark navigation, map-matching). 
% SLAM \cite{durrant2006simultaneous1, bailey2006simultaneous2}. 
% Trilateration in robotics \cite{thomas2005revisiting}
% Improved Grid Mapping with Rao-Blackwellized particle filters \cite{grisetti2007improved}. 
% Map representations depend on the nature of the environment and the problem, and include landmark-based maps, occupancy grid maps, and object/polygon maps \cite{thrun2002robotic}.

In the multi-robot system literature, several approaches extend single-robot SLAM to allow each robot to compute a map, broadcast map updates, and localize within the joint map when possible \cite{thrun2001probabilistic, li2017corb, liu2013fast}. 
% This requires known initial positions, or for all robots but one to initialize by localizing within the map of the first. 
Efforts to coordinate multi-robot systems in unknown environment exploration are commonly focused on increasing efficiency by minimizing the total time to cover an area \cite{simmons2000coordination, burgard2005coordinated, valencia2018active}. Previous work has focused on improving particle filter localization in multi-robot systems with relative position estimates \cite{fox1999collaborative}, however these robots rely on visual perception and laser rangefinder distances for relative positioning, and do not rely on explicit communication.
% SLAM for teams, same basic algorithm but map updates broadcasted \cite{thrun2001probabilistic}, requires known initial positions or that all robots start within the map of one robot.
% coordination to minimize time needed to map \cite{simmons2000coordination, burgard2005coordinated}.
% Improved monte carlo localization with relative position estimates based on visual perception and laser rangefinder distances (without explicit communication) \cite{fox1999collaborative}.
Recently, the use of ultra-wideband technology for robot positioning has received some attention. These largely fall into three categories: infrastructure-based UWB positioning with known anchor locations \cite{fan2017data, zhang2018linear, song2019uwb, liu2018multi}, UWB positioning within a known map \cite{park2016bim}, or relative positioning for the purpose of formation control or leader-follower control \cite{qiang2018formation, nguyen2019distance}. Previous work using multi-robot trilateration is presented in \cite{ maxim2008trilateration}. Add something here.

Localization is also a popular research topic in wireless sensor networks where resources are often more limited \cite{peralta2007collaborative, mao2007wireless}. 
% Sensor localization algorithms can be classified as either range-based (using distance estimates) \cite{ahmadi2017exploiting} or range-free (using connectivity data to establish neighbors and infer positions) \cite{ahmadi2016range}. 
% Solutions can further be
Sensor localization algorithms can be categorized as anchor-based or recursive, repeatedly applying the basic algorithm and converting ordinary nodes to anchor nodes after their position is determined \cite{kirci2016recursive, bouhdid2020low}. 
% Some approaches rely on multi-dimensional scaling, a statistical technique for arranging nodes in an n-dimensional space based on distances between the nodes \cite{chaurasiya2014novel}.
% Node mobility can be used to assist localization through dynamic repositioning for connectivity maintenance or using some mobile nodes in a static network to increase density in sparse areas \cite{wu2006mobile}.
Mobile anchor nodes can be used to assist localization in wireless sensor networks \cite{han2016survey}. Conversely, sensor networks can also aid localization for mobile/robotic nodes \cite{taylor2005simultaneous, djugash2006range, fu2010local}. In this work we take a recursive trilateration approach to localization and further address the challenges specific to robotic networks exploration, including mobility and mapping.

%  To the best of our knowledge, this work is the first to approach multi-robot exploration and mapping with infrastructure-less UWB positioning.
% Infrastructure-based: \cite{fan2017data, zhang2018linear, song2019uwb, liu2018multi}
% Known maps: \cite{park2016bim}
% For formation control or leader-follower: \cite{qiang2018formation, nguyen2019distance}
% Other methods of multi-robot trilateration for localization, which do not approach mapping: \cite{ maxim2008trilateration}

% While extensive experimental research exists in both robotic exploration and wireless sensor networks, real-world experiments at the intersection of these fields
% Briefly, we note that relevant literature exists on the design and implementation of robotic network testbeds and mobile ad-hoc network testbeds \cite{jimenez2013testbeds, tran2018intelligent, farkhana2018mobility}.
% Robotic network testbeds
% A comprehensive survey on robot network testbeds \cite{jimenez2013testbeds}
% Our previous work on robotic wireless network testbed \cite{tran2018intelligent}
% A more recent survey on mobile ad-hoc network testbeds \cite{farkhana2018mobility}

